GalSyn I: A Forward-Modeling Code for Synthetic Galaxy Observations from Hydrodynamical Simulations and First Data Release from IllustrisTNG

We present GalSyn (Galaxy Synthesizer), a modular and flexible Python package for generating synthetic observations from hydrodynamical galaxy simulations. GalSyn generates synthetic spectrophotometric data cubes for individual galaxies from simulation cutouts, employing a particle-by-particle spectral modeling approach that enables the rapid production of large synthetic datasets required for statistical population studies, offering a computationally efficient alternative to full radiative transfer codes. Users have full control over the spectral modeling choices, including the stellar population synthesis engine, stellar isochrones, spectral libraries, and initial mass functions. Dust attenuation is modeled at spatially resolved scales using a line-of-sight column-density method, with a comprehensive suite of fixed and adaptive attenuation laws. A decoupled kinematics model independently Doppler-shifts the stellar and nebular components, enabling realistic synthetic integral field unit data cubes. It also provides features to add observational realism, including PSF convolution and noise simulation. Beyond generating imaging and spectroscopic data cubes, GalSyn reconstructs spatially resolved physical property maps and star formation histories (SFHs) of a galaxy. Alongside this paper, we present the first data release of synthetic imaging observations and resolved SFHs generated from the IllustrisTNG simulations. This release includes four mock extragalactic survey fields together with data cubes of the individual galaxies within them, data cubes of 290 local massive galaxies and their progenitors tracked across $0<z<5$, and 259 major-merger systems. Each galaxy data cube contains imaging across 47 filters spanning HST, JWST, Euclid, Rubin/LSST, and the Roman Space Telescope. GalSyn is publicly available at https://github.com/aabdurrouf/GalSyn.

==> tab_noise_sim_params.tex <==
\begin{table}[ht]
\centering
\caption{Input parameters for simulating noise in \galsyn.}
\renewcommand{\arraystretch}{1.5} % Increase row spacing for readability
\begin{tabularx}{\textwidth}{@{} >{\raggedright}p{3cm} X >{\raggedright}p{3cm} >{\raggedright\arraybackslash}p{3cm} @{}}
\toprule
\textbf{Conceptual Parameter} & \textbf{Description} & \textbf{Imaging Implementation} & \textbf{IFU Implementation} \\
\midrule
\textbf{Magnitude Zero-Point} & The instrumental magnitude used to convert between magnitudes and detected counts. & \textbf{Name:} \texttt{mag\_zp} \newline \textbf{Type:} Dictionary & \textbf{Name:} \texttt{mag\_zp} \newline \textbf{Type:} Float or Callable \\
\addlinespace
\textbf{Limiting Magnitude} & The magnitude of the faintest source detectable at a given S/N, defining the observation's depth. & \textbf{Name:} \texttt{limiting\_magnitude} \newline \textbf{Type:} Dictionary & \textbf{Name:} \texttt{limiting\_magnitude\_wave\_func} \newline \textbf{Type:} Callable \\
\addlinespace
\textbf{Signal-to-Noise Ratio} & The S/N achieved for a source at the specified limiting magnitude. & \textbf{Name:} \texttt{snr\_limit} \newline \textbf{Type:} Dictionary & \textbf{Name:} \texttt{snr\_limit} \newline \textbf{Type:} Float or Callable \\
\addlinespace
\textbf{Exposure Time} & The total integration time of the observation in seconds. & \textbf{Name:} \texttt{exposure\_time} \newline \textbf{Type:} Dictionary & \textbf{Name:} \texttt{exposure\_time} \newline \textbf{Type:} Float or Callable \\
\addlinespace
\textbf{Aperture Radius} & The radius of the circular aperture (in arcseconds) within which the limiting magnitude is defined. & \textbf{Name:} \texttt{aperture\_radius\_arcsec} \newline \textbf{Type:} Dictionary & Not Applicable \\
\bottomrule
\end{tabularx}
\footnotesize{%
\textbf{Note on Data Types:} \\
\textbf{Dictionary:} For imaging, parameters are dictionaries keyed by filter name (e.g., \texttt{'jwst\_f200w'}). \\
\textbf{Float or Callable:} For IFU data, parameters can be a single number (Float) for all wavelengths or a function (Callable) that returns a value for a given wavelength, allowing for spectrally-dependent noise characteristics.
}
\end{table}
